Imbalanced malware classification: an approach based on dynamic classifier selection

In recent years, the rise of cyber threats has emphasized the need for robust malware detection systems, especially on mobile devices. Malware, which targets vulnerabilities in devices and user data, represents a substantial security risk. A significant challenge in malware detection is the imbalance in datasets, where most applications are benign, with only a small fraction posing a threat. This study addresses the often-overlooked issue of class imbalance in malware detection by evaluating various machine learning strategies for detecting malware in Android applications. We assess monolithic classifiers and ensemble methods, focusing on dynamic selection algorithms, which have shown superior performance compared to traditional approaches. In contrast to balancing strategies performed on the whole dataset, we propose a balancing procedure that works individually for each classifier in the pool. Our empirical analysis demonstrates that the KNOP algorithm obtained the best results using a pool of Random Forest. Additionally, an instance hardness assessment revealed that balancing reduces the difficulty of the minority class and enhances the detection of the minority class (malware). The code used for the experiments is available at https://github.com/jvss2/Machine-Learning-Empirical-Evaluation.

==> tables/Balanced_metrics.tex <==
\begin{table*}[p]
    \centering
    \renewcommand{\arraystretch}{1.2}
    \caption{\textbf{Performance metrics of various classifiers on balanced data.} Recall, F1 Score, ROC AUC, G-Mean, and MCC for each model, with standard deviations shown in parentheses. Color coding highlights the top three performances: red indicates the best, blue the second best, and burgundy the third.}
    \label{tab:Balanced_metrics}
    \begin{tabular}{l|l|l|l|l|l}
    \toprule
Model               & Recall                              & F1 score       & AUC        & G-Mean         & MCC            \\
\midrule             

DecisionTree        & 86.11(00.82)                      & 71.02(00.32) & 91.78(00.37) & 91.61(00.40) & 70.69(00.29) \\

KNN                 & \textcolor{purple}{89.30(00.82)}  & 63.93(00.54) & 92.62(00.37) & 92.56(00.38) & 64.82(00.47) \\

MLP                 & 88.55(01.63)                      & 53.28(03.12) & 91.01(00.46) & 90.96(00.48) & 55.53(02.43) \\

NaiveBayes          & 73.72(03.73)                      & 18.85(00.27) & 73.16(01.12) & 73.11(01.13) & 20.65(00.71) \\

\hline               

BaggingDT           & 87.16(00.79)                      & 75.77(00.89) & 92.61(00.39) & 92.45(00.42) & 75.24(00.88) \\

BaggingKNN          & \textcolor{red}{90.75(00.82)}     & 60.93(00.56) & \textcolor{blue}{92.96(00.40)} & \textcolor{red}{92.93(00.41)} & 62.48(00.56) \\

BaggingMLP          & \textcolor{blue}{90.18(00.72)}    & 57.15(00.69) & 92.27(00.38) & 92.24(00.38) & 59.14(00.68) \\

BaggingNB           & 74.33(02.75)                      & 18.87(00.49) & 73.34(01.01) & 73.31(01.01) & 20.77(00.83) \\

\hline              

baggingDT-2         & 86.00(00.35)                      & 81.64(00.52) & 92.44(00.18) & 92.22(00.19) & 80.88(00.52) \\

baggingKNN-2        & 88.99(00.46)                      & 69.69(00.31) & \textcolor{red}{93.00(00.22)} & \textcolor{blue}{92.91(00.23)} & 69.87(00.32) \\

baggingMLP-2        & 88.80(01.09) & 59.93(01.00) &91.98(00.54) &91.92(00.56) &61.26(00.97) \\

baggingNB-2         & 73.97(00.21)                      & 18.70(00.20) & 73.09(00.14) & 73.08(00.15) & 20.51(00.21) \\

\hline       

GBDT                & 86.65(01.37)                      & 42.04(00.73) & 88.24(00.68) & 88.23(00.69) & 45.52(00.83) \\

RandomForest        & 87.40(00.89)                      & 79.13(00.84) & \textcolor{purple}{92.94(00.44)} & \textcolor{purple}{92.78(00.47)} & 78.49(00.85) \\

SingleBest          & 86.89(00.96)                      & 67.01(00.88) & 91.81(00.47) & 91.68(00.50) & 67.16(00.86) \\

StaticSelection     & 87.19(00.91)                      & 79.41(00.81) & 92.87(00.44) & 92.69(00.47) & 78.74(00.82) \\

\hline

%SingleBest-2 & 83.23(01.19) & 67.89(01.06) & 90.22(00.60) & 89.95(00.65) & 67.46(01.06)\\

%StaticSelection-2 & 85.56(00.89) & \textcolor{purple}{82.24(00.58)} & 92.27(00.43) & 92.03(00.47) & \textcolor{purple}{81.48(00.60)}\\

\hline

KNOP                & 85.77(01.07)                      & 81.19(00.83) & 92.31(00.52) & 92.07(00.56) & 80.42(00.86) \\

METADES             & 85.26(01.14)                      & 80.14(00.80) & 92.01(00.55) & 91.76(00.60) & 79.35(00.83) \\

OLA                 & 86.99(00.99)                      & 70.26(00.90) & 92.13(00.50) & 91.98(00.53) & 70.10(00.91) \\

\hline

OLA-2 & 84.85(01.00) & 74.59(00.75) & 91.46(00.48) & 91.22(00.52) & 73.91(00.76) \\

KNOP-2 & 84.32(01.07) & \textcolor{red}{84.58(00.87)} & 91.82(00.51) & 91.51(00.55) & \textcolor{red}{83.91(00.92)} \\

METADES-2 & 83.47(01.27) & \textcolor{blue}{83.40(00.84)} & 91.36(00.60) & 91.01(00.67) & \textcolor{blue}{82.67(00.88)}\\
\bottomrule 
\end{tabular}

\end{table*}

==> tables/Imbalanced_metrics.tex <==
\begin{table*}[!h]
    \centering
    \renewcommand{\arraystretch}{1.2}
    \setlength{\tabcolsep}{5pt}
    \caption{\textbf{Performance metrics of various classifiers on imbalanced data.} Recall, F1 Score, ROC AUC, G-Mean, and MCC for each model, with standard deviations shown in parentheses. Color coding highlights the top three performances: red indicates the best, blue the second best, and burgundy the third.}
    \label{tab:Imbalanced_metrics}
    \begin{tabular}{l|l|l|l|l|l}
\toprule
Model           & Recall                              & F1 score                            & AUC                           & G-Mean                          & MCC                                   \\
\midrule
DecisionTree    &  \textcolor{red}{82.24(01.19)}    & 79.65(00.94)                      &  \textcolor{red}{90.57(00.60)}    &  \textcolor{red}{90.19(00.65)}    & 78.75(00.98)                      \\
KNN             & 73.42(01.70)                      & 77.11(01.20)                      & 86.33(00.85)                      & 85.35(00.99)                      & 76.25(01.23)                      \\
MLP             & 59.26(04.40)                      & 68.51(02.38)                      & 79.32(02.13)                      & 76.69(02.85)                      & 68.37(01.89)                      \\
NaiveBayes      & 46.27(01.77)                      & 32.52(01.18)                      & 70.02(00.86)                      & 65.86(01.23)                      & 30.06(01.27)                      \\
\hline
BaggingDT       &  \textcolor{purple}{81.15(01.08)}   & 85.07(00.67)                      &  \textcolor{blue}{90.36(00.53)}   &  \textcolor{blue}{89.89(00.59)}   & 84.54(00.69)                      \\
BaggingKNN      & 73.19(01.31)                      & 77.36(01.04)                      & 86.23(00.65)                      & 85.24(00.76)                      & 76.54(01.08)                      \\
BaggingMLP      & 60.76(01.71)                      & 71.17(01.17)                      & 80.15(00.85)                      & 77.76(01.09)                      & 71.26(01.07)                      \\
BaggingNB       & 46.53(01.23)                      & 32.83(00.81)                      & 70.18(00.59)                      & 66.07(00.85)                      & 30.38(00.87)                      \\
\hline
GBDT            & 46.93(02.04)                      & 60.29(01.83)                      & 73.27(01.02)                      & 68.36(01.49)                      & 61.78(01.63)                      \\
RandomForest    & 80.45(01.28)                      & 86.43(00.84)                      & 90.10(00.64)                      & 89.58(00.71)                      & 86.12(00.84)                      \\
SingleBest      & 79.00(01.03)                      & 77.71(00.79)                      & 88.95(00.51)                      & 88.39(00.57)                      & 76.71(00.83)                      \\
StaticSelection & 80.39(01.12)                      &  \textcolor{purple}{86.52(00.78)} & 90.07(00.56)                      & 89.55(00.62)                      &  \textcolor{purple}{86.24(00.79)} \\
\hline
KNOP            & 80.49(01.11)                      &  \textcolor{red}{86.69(00.68)}    & 90.13(00.55)                      & 89.61(00.62)                      &  \textcolor{red}{86.43(00.68)}    \\
METADES         &  80.92(01.06) &  \textcolor{blue}{86.60(00.63)}   &  \textcolor{purple}{90.33(00.52)} & 89.83(00.58)                      &  \textcolor{blue}{86.27(00.64)}   \\
OLA             & \textcolor{blue}{81.57(00.96)}                      & 80.10(00.70)                      & 90.29(00.47)                      &  \textcolor{purple}{89.87(00.52)} & 79.21(00.73)                      \\

\bottomrule
\end{tabular}
\end{table*}

==> tables/hiperparameters.tex <==
\begin{table}
\centering
\caption{Classifier Hyperparameters}\label{tb:hiperparameters}
\begin{tabular}{l l}
\toprule
Classifiers & Hyperparameters\\
\midrule
Decision Tree & Criterion = Gini\\
KNN & k = 7\\ 
MLP & n\_hidden = (100), max\_iter = 1000\\
Naive Bayes & Algorithm = Gaussian\\
\hline
Bagging (DT, KNN, MLP, NB) &  n\_estimators = 100\\
\hline
Gradient Boosted Decision Tree & n\_estimators = 100\\
Random Forest & n\_estimators = 100\\
SingleBest & score function = accuracy\\
StaticSelection & score function = accuracy\\
\hline
KNOP & k = 7\\
METADES & k = 7, selection threshold = 0.5\\
OLA & k = 7\\
\bottomrule
\end{tabular}
\end{table}


==> tables/name.tex <==
\begin{table*}[p]
    \centering
    \renewcommand{\arraystretch}{1.2}
    \caption{\textbf{Evolution After Balancing.} Recall, F1 Score, ROC AUC, G-Mean, and MCC for each model, with standard deviations shown in parentheses. Color coding highlights the top three performances: red indicates the best, blue the second best, and burgundy the third.}
    \label{tab:comparison}
    \begin{tabular}{l|l|l|l|p{0.7cm}|l}
\toprule
Model                       &Recall & F1 score & G-Mean & ROC AUC & MCC     \\
\midrule            
DecisionTree                &03.86 & -08.63  & 01.42 & 01.21  & -08.06 \\
KNN                         &15.88 & -13.18  & 07.21 & 06.29  & -11.43 \\
MLP                         &\textcolor{purple}{29.29} & -15.22  &  \textcolor{purple}{14.28} & 11.68  & -12.84 \\
NaiveBayes                  &27.45 & -13.67  & 07.25 & 03.14  & -09.40 \\
\hline                      
BaggingDeT         &06.01 & -09.30  & 02.57 & 02.26  & -09.30 \\
BaggingKNN                  &17.56 & -16.43  & 07.70 & 06.73  & -14.07 \\
BaggingMLP                  &\textcolor{blue}{29.42} & -14.02  & \textcolor{blue}{14.48} & \textcolor{blue}{12.11}  & -12.12 \\
BaggingNB          & 27.80 & -13.96  & 07.24 & 03.16  & -09.61 \\
\hline                      
baggingDT-2      & 04.84 & \textcolor{red}{-03.43}  & 02.33 & 02.08  & \textcolor{red}{-03.66} \\
baggingKNN-2                &15.80 & -07.67  & 07.68 & 06.77  & \textcolor{purple}{-06.68} \\
baggingMLP-2               & 28.04 & -11.24  & 14.16 & \textcolor{purple}{11.83}  & -01.00 \\
baggingNB-2        & 27.44 & -14.13  & 07.01 & 02.91  & -09.87 \\
\hline                      
GBDT                        & \textcolor{red}{39.72} & -18.25  & \textcolor{red}{19.87} & \textcolor{red}{14.97}  & -16.26 \\
RandomForest                &06.95 & -07.30  & 03.20 & 02.85  & -07.64 \\
SingleBest                  &07.89 & -10.70  & 03.29 & 02.86  & -09.54 \\
StaticSelection             &06.80 & -07.11  & 03.14 & 02.79  & -07.49 \\
\hline   
KNOP                        &05.28 & \textcolor{blue}{-05.51}  & 02.47 & 02.18  & \textcolor{blue}{-06.00} \\
METADES                     &04.34 & \textcolor{purple}{-06.46}  & 01.93 & 01.68  & -06.92 \\
OLA                         &05.41 & -09.84  & 02.12 & 01.84  & -09.10 \\
\bottomrule         
\end{tabular}
\label{tab:resultados_modelos}
\end{table*}

==> tables/name1.tex <==
\begin{table*}[p]
    \centering
    \setlength{\tabcolsep}{5pt}  
    \large 
\renewcommand{\arraystretch}{1.2}
    \caption{\textbf{Performance metrics of various classifiers on imbalanced and balanced data.} Recall, F1 Score, ROC AUC, G-Mean, and MCC for each model, with standard deviations shown in parentheses. Color coding highlights the top three performances: red indicates the best, blue the second best, and burgundy the third.}
    \label{tab:Combined_metrics}
    \resizebox{\textwidth}{!}{ 
    \begin{tabular}{l|lllll|lllll}
    \toprule

\textbf{Model} & \multicolumn{5}{c|}{\textbf{Imbalanced}} & \multicolumn{5}{c}{\textbf{Balanced}} \\
               & \textbf{Recall} & \textbf{F1 score} & \textbf{ROC AUC} & \textbf{G-Mean} & \textbf{MCC} & \textbf{Recall} & \textbf{F1 score} & \textbf{ROC AUC} & \textbf{G-Mean} & \textbf{MCC} \\
    \midrule
DecisionTree    &  \textcolor{red}{82.24(01.19)}             & 79.65(00.94)                       &  \textcolor{red}{90.57(00.60)}    &  \textcolor{red}{90.19(00.65)}    & 78.75(00.98)   & 86.11(00.82)                          & 71.02(00.32)                       & 91.78(00.37)                      & 91.61(00.40)                      & 70.69(00.29)  \\
KNN             & 73.42(01.70)                              & 77.11(01.20)                       & 86.33(00.85)                      & 85.35(00.99)                      & 76.25(01.23)   & \textcolor{purple}{89.30(00.82)}      & 63.93(00.54)                       & 92.62(00.37)                      & 92.56(00.38)                      & 64.82(00.47) \\
MLP             & 59.26(04.40)                              & 68.51(02.38)                       & 79.32(02.13)                      & 76.69(02.85)                      & 68.37(01.89)   & 88.55(01.63)                          & 53.28(03.12)                       & 91.01(00.46)                      & 90.96(00.48)                      & 55.53(02.43) \\
NaiveBayes      & 46.27(01.77)                              & 32.52(01.18)                       & 70.02(00.86)                      & 65.86(01.23)                      & 30.06(01.27)   & 73.72(03.73)                          & 18.85(00.27)                       & 73.16(01.12)                      & 73.11(01.13)                      & 20.65(00.71) \\
\hline
BaggingDT       &  \textcolor{purple}{81.15(01.08)}         & 85.07(00.67)                       &  \textcolor{blue}{90.36(00.53)}   &  \textcolor{blue}{89.89(00.59)}   & 84.54(00.69)   & 87.16(00.79)                          & 75.77(00.89)                       & 92.61(00.39)                      & 92.45(00.42)                      & 75.24(00.88) \\
BaggingKNN      & 73.19(01.31)                              & 77.36(01.04)                       & 86.23(00.65)                      & 85.24(00.76)                      & 76.54(01.08)   & \textcolor{red}{90.75(00.82)}         & 60.93(00.56)                       & \textcolor{blue}{92.96(00.40)}     & \textcolor{red}{92.93(00.41)}     & 62.48(00.56) \\
BaggingMLP      & 60.76(01.71)                              & 71.17(01.17)                       & 80.15(00.85)                      & 77.76(01.09)                      & 71.26(01.07)   & \textcolor{blue}{90.18(00.72)}        & 57.15(00.69)                       & 92.27(00.38)                      & 92.24(00.38)                      & 59.14(00.68) \\
BaggingNB       & 46.53(01.23)                              & 32.83(00.81)                       & 70.18(00.59)                      & 66.07(00.85)                      & 30.38(00.87)   & 74.33(02.75)                          & 18.87(00.49)                       & 73.34(01.01)                      & 73.31(01.01)                      & 20.77(00.83) \\
\hline
baggingDT-2   & - & - & - & - & -      & 86.00(00.35)                      & 81.64(00.52) & 92.44(00.18) & 92.22(00.19) & 80.88(00.52) \\

baggingKNN-2   & - & - & - & - & -     & 88.99(00.46)                      & 69.69(00.31) & \textcolor{red}{93.00(00.22)} & \textcolor{blue}{92.91(00.23)} & 69.87(00.32) \\

baggingMLP-2   & - & - & - & - & -     & 88.80(01.09) & 59.93(01.00) &91.98(00.54) &91.92(00.56) &61.26(00.97) \\

baggingNB-2   & - & - & - & - & -      & 73.97(00.21)                      & 18.70(00.20) & 73.09(00.14) & 73.08(00.15) & 20.51(00.21) \\

\hline       

GBDT            & 46.93(02.04)                              & 60.29(01.83)                       & 73.27(01.02)                      & 68.36(01.49)                      & 61.78(01.63)   & 86.65(01.37)                          & 42.04(00.73)                       & 88.24(00.68)                      & 88.23(00.69)                      & 45.52(00.83) \\
RandomForest    & 80.45(01.28)                              & 86.43(00.84)                       & 90.10(00.64)                      & 89.58(00.71)                      & 86.12(00.84)   & 87.40(00.89)                          & 79.13(00.84)                       & \textcolor{purple}{92.94(00.44)}   & \textcolor{purple}{92.78(00.47)}   & 78.49(00.85) \\
SingleBest      & 79.00(01.03)                              & 77.71(00.79)                       & 88.95(00.51)                      & 88.39(00.57)                      & 76.71(00.83)   & 86.89(00.96)                          & 67.01(00.88)                       & 91.81(00.47)                      & 91.68(00.50)                      & 67.16(00.86) \\
StaticSelection & 80.39(01.12)                              &  \textcolor{purple}{86.52(00.78)}  & 90.07(00.56)                      & 89.55(00.62)                      &  \textcolor{purple}{86.24(00.79)}  & 87.19(00.91)                          & 79.41(00.81)                       & 92.87(00.44)                      & 92.69(00.47)                      & 78.74(00.82) \\
\hline
KNOP            & 80.49(01.11)                              &  \textcolor{red}{86.69(00.68)}     & 90.13(00.55)                      & 89.61(00.62)                      &  \textcolor{red}{86.43(00.68)}     & 87.41(00.93)                          & \textcolor{red}{80.24(00.73)}       & \textcolor{red}{92.99(00.44)}      & \textcolor{blue}{92.81(00.47)}     & \textcolor{blue}{79.77(00.75)} \\
METADES         &  80.92(01.06)                             &  \textcolor{blue}{86.60(00.63)}   &  \textcolor{purple}{90.33(00.52)} & 89.83(00.58)                      &  \textcolor{blue}{86.27(00.64)}    & 87.34(00.94)                          & \textcolor{blue}{79.73(00.76)}      & 92.92(00.43)                      & \textcolor{purple}{92.79(00.46)}   & \textcolor{purple}{79.38(00.77)} \\
OLA             & \textcolor{blue}{81.57(00.96)}                              & 80.10(00.70)                       & 90.29(00.47)                      & \textcolor{purple}{89.87(00.52)}                      & 79.21(00.73)   & 87.12(01.09)                          & 72.44(00.63)                       & 92.84(00.52)                      & 92.68(00.55)                      & 73.18(00.61) \\
\hline

OLA-2 & - & - & - & - & - & 84.85(01.00) & 74.59(00.75) & 91.46(00.48) & 91.22(00.52) & 73.91(00.76) \\

KNOP-2 & - & - & - & - & - & 84.32(01.07) & \textcolor{red}{84.58(00.87)} & 91.82(00.51) & 91.51(00.55) & \textcolor{red}{83.91(00.92)} \\

METADES-2 & - & - & - & - & - & 83.47(01.27) & \textcolor{blue}{83.40(00.84)} & 91.36(00.60) & 91.01(00.67) & \textcolor{blue}{82.67(00.88)}\\
\bottomrule
\end{tabular}
}
\end{table*}

